The Photometric LSST Astronomical Time-series Classification Challenge (PLAsTiCC): Selection of a performance metric for classification probabilities balancing diverse science goals

Classification of transient and variable light curves is an essential step in using astronomical observations to develop an understanding of their underlying physical processes. However, upcoming deep photometric surveys, including the Large Synoptic Survey Telescope (LSST), will produce a deluge of low signal-to-noise data for which traditional labeling procedures are inappropriate. Probabilistic classification is more appropriate for the data but are incompatible with the traditional metrics used on deterministic classifications. Furthermore, large survey collaborations intend to use these classification probabilities for diverse science objectives, indicating a need for a metric that balances a variety of goals. We describe the process used to develop an optimal performance metric for an open classification challenge that seeks probabilistic classifications and must serve many scientific interests. The Photometric LSST Astronomical Time-series Classification Challenge (PLAsTiCC) is an open competition aiming to identify promising techniques for obtaining classification probabilities of transient and variable objects by engaging a broader community both within and outside astronomy. Using mock classification probability submissions emulating archetypes of those anticipated of PLAsTiCC, we compare the sensitivity of metrics of classification probabilities under various weighting schemes, finding that they yield qualitatively consistent results. We choose as a metric for PLAsTiCC a weighted modification of the cross-entropy because it can be meaningfully interpreted. Finally, we propose extensions of our methodology to ever more complex challenge goals and suggest some guiding principles for approaching the choice of a metric of probabilistic classifications.

==> authors.tex <==
% Author list file generated with: mkauthlist 1.2.3
% mkauthlist -j apj -f -c the LSST Dark Energy Science Collaboration \ and \ the LSST Transients and Variable Stars Science Collaboration --cntrb contributions.tex authors.csv authors.tex

\author{A.I.~Malz}
\affiliation{German Centre of Cosmological Lensing, Ruhr-Universit\"{a}t Bochum, Universit\"{a}tsstra{\ss}e 150, 44801 Bochum, Germany}
\affiliation{Center for Cosmology and Particle Physics, New York University, 726 Broadway, New York, NY 10004, USA}
\affiliation{Department of Physics, New York University, 726 Broadway, New York, NY 10004, USA}
\author{R.~Hlo\v{z}ek}
\affiliation{Department of Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\affiliation{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{T.~Allam Jr}
\affiliation{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Holmbury Hill Rd, Dorking RH5 6NT, UK}
\author{A.~Bahmanyar}
\affiliation{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{R.~Biswas}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\author{M.~Dai}
\affiliation{Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854 USA}
\author{L.~Galbany}
\affiliation{University of Pittsburgh, 300 Allen Hall, 3941 O'Hara St, Pittsburgh, PA 15260}
\author{E.E.O.~Ishida}
\affiliation{Universit\'e Clermont Auvergne, CNRS/IN2P3, LPC, F-63000 Clermont-Ferrand, France}
\author{S.W.~Jha}
\affiliation{Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854 USA}
\author{D.~Jones}
\affiliation{University of Santa Cruz, 1156 High St, Santa Cruz, CA 95064, USA}
\author{R.~Kessler}
\affiliation{KICP, 5640 S Ellis Ave, Chicago, IL 60637}
\author{M.~Lochner}
\affiliation{African Institute for Mathematical Sciences, 6 Melrose Road, Muizenberg, 7945, South Africa}
\affiliation{South African Radio Astronomy Observatory, The Park, Park Road, Pinelands, Cape Town 7405, South Africa}
\author{A.A.~Mahabal}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{Center for Data Driven Discovery, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.S.~Mandel}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation{Statistical Laboratory, DPMMS, University of Cambridge, Wilberforce Road, Cambridge, CB3 0WB, UK}
\author{J.R.~Mart\'inez-Galarza}
\affiliation{Harvard-Smithsonian Center for Astrophysics, 60 Garden Street,Mail Stop 66 Cambridge, MA 02138}
\author{J.D.~McEwen}
\affiliation{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Holmbury Hill Rd, Dorking RH5 6NT, UK}
\author{D.~Muthukrishna}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\author{G.~Narayan}
\affiliation{Space Telescope Science Institute, 3700 San Martin Dr, Baltimore, MD 21218, USA}
\author{H.~Peiris}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{C.M.~Peters}
\affiliation{Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{K.~Ponder}
\affiliation{Berkeley Center for Cosmological Physics, Campbell Hall 341, University of California Berkeley, Berkeley, CA 94720, USA}
\author{C.N.~Setzer}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}


\collaboration{(the LSST Dark Energy Science Collaboration \ and \ the LSST Transients and Variable Stars Science Collaboration)}

